Is Large Language Model Performance on Reasoning Tasks Impacted by Different Ways Questions Are Asked?

Large Language Models (LLMs) have been evaluated using diverse question types, e.g., multiple-choice, true/false, and short/long answers. This study answers an unexplored question about the impact of different question types on LLM accuracy on reasoning tasks. We investigate the performance of five LLMs on three different types of questions using quantitative and deductive reasoning tasks. The performance metrics include accuracy in the reasoning steps and choosing the final answer. Key Findings: (1) Significant differences exist in LLM performance across different question types. (2) Reasoning accuracy does not necessarily correlate with the final selection accuracy. (3) The number of options and the choice of words, influence LLM performance.

==> latex/unused_sentences.tex <==
\iffalse
We conduct experiments using three different LLMs on two different datasets, and the three different types of questions are applied for every question. For each question, we calculate two metrics: final selection accuracy and reasoning accuracy. Greedy decoding is utilized for generating responses, but due to the variability of LLMs accuracy fluctuates across trials. To address this, we apply the Wilcoxon signed-rank test to assess if the differences in accuracy across question types are statistically significant. The distributions of annotated outputs, which contain 0 (incorrect) and 1 (correct) are compared.
\fi
